Vid2Seq: Large-Scale Pretraining of a Visual Language Model for Dense Video Captioning

In this work, we introduce Vid2Seq, a multi-modal single-stage dense event captioning model pretrained on narrated videos which are readily-available at scale. The Vid2Seq architecture augments a language model with special time tokens, allowing it to seamlessly predict event boundaries and textual descriptions in the same output sequence. Such a unified model requires large-scale training data, which is not available in current annotated datasets. We show that it is possible to leverage unlabeled narrated videos for dense video captioning, by reformulating sentence boundaries of transcribed speech as pseudo event boundaries, and using the transcribed speech sentences as pseudo event captions. The resulting Vid2Seq model pretrained on the YT-Temporal-1B dataset improves the state of the art on a variety of dense video captioning benchmarks including YouCook2, ViTT and ActivityNet Captions. Vid2Seq also generalizes well to the tasks of video paragraph captioning and video clip captioning, and to few-shot settings. Our code is publicly available at https://antoyang.github.io/vid2seq.html.

==> bin.tex <==
\begin{table}[t]
\begin{center}
\setlength\tabcolsep{1pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|cc|cc|cc}
& \multirow{2}{*}{Method}
& \multicolumn{2}{c|}{YouCook2 (val)}
& \multicolumn{2}{c|}{ViTT (test)}
& \multicolumn{2}{c}{MSR-VTT (test)} \\
& & \small{CIDEr} & \small{METEOR} & \small{CIDEr} & \small{METEOR} & \small{CIDEr} & \small{METEOR} \\
\hline
1. & M-MASS~\cite{huang2020multimodal}
& 123 & 18.3 & 82 & 11.0 & --- & --- \\
2. & DECEMBERT~\cite{tang2021decembert}
& 58 & 20.0 & --- & --- & 52 & 29.7 \\
3. & UniVL~\cite{luo2020univilm}
& 181 & 22.4 & --- & --- & 50 & 28.9 \\
4. & SwinBERT~\cite{lin2022swinbert} & 109.0 & 15.6 & --- & --- & 53.8 & 29.9 \\
5. & MV-GPT~\cite{seo2022end}
& 221 & ---$^*$ & 104 & ---$^*$ & 60 & ---$^*$ \\
6. & \model{} (Ours) 
& \textbf{247.8} & \textbf{25.1} & \textbf{221.3} & \textbf{26.9} & \textbf{61.4} & \textbf{30.3} \\
\end{tabular}
}
\end{center}
\vspace{-0.7cm}
\caption{\small Comparison to the SoTA for video clip captioning.
* Authors confirmed that they used an incorrect metric implementation.}  
\vspace{-0.7cm}
\label{table:sotaclip}
\end{table}

\begin{table*}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{6pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc|ccccc}
& \makecell{\small{Visual} \\
\small{Temporal Embedding}} & \makecell{\small{Speech} \\
\small{Time Tokens}}  &
\multicolumn{5}{c|}{YouCook2 (val)} &
\multicolumn{5}{c}{ActivityNet Captions (val)} \\
& & & \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} 
& \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} \\ 
\hline
1. & \xmark & \xmark
& X & X & X & X & X
& X & X & X & X & X \\
2. & \cmark & \xmark
& X & X & X & X & X
& X & X & X & X & X \\
3. & \xmark & \cmark
& 6.8 & 42.0 & 8.6 & 26.7 & 24.6
& 5.3 & 27.0 & 7.8 & 50.6 & 53.2 \\ 
4. & \cmark & \cmark
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3} & \textbf{27.9} & \textbf{27.8} 
& 5.8 & 30.1 & \textbf{8.5} & \textbf{52.7} & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on the time encodings in our model.}
\vspace{-0.7cm}
\label{table:time}
\end{center}
\end{table*}



\noindent \textbf{Impact of modalities and pretraining objectives.} 
Table \ref{table:modalities}
Repretrain w/o time encodings, w/o time tokens

\noindent \textbf{Impact of the language model initialization.} 
Table \ref{table:language}
Repretrain w/o LM init

\noindent \textbf{Interaction between localization and captioning.} 
The following studies are true on YouCook2 but not on ActivityNet.

Table \ref{table:twostage}.
Use the same models and explain the 2-stage is tuned as best as possible.
Better localization so captioning helps localizing.

Table \ref{table:time}.
Use the previous models.
Better captioning so localization helps captioning.

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{cccc|ccccc}
& Denoising & \multicolumn{2}{c|}{Generative} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
& & \small{video-level} & \small{clip-level} & & & & \\ 
\hline
1. & \xmark & \xmark & \xmark
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3 \\ 
2. & \cmark & \xmark & \xmark
& 7.9 & 47.6 & 9.7 & 27.2 & 28.0 \\ 
3. & \xmark & \cmark & \xmark
& 5.7 & 25.3 & 6.1 & 24.4 & 23.6 \\ %
4. & \cmark & \xmark & \cmark
& 8.0 & 47.2 & 9.6 & 27.2 & 28.3 \\
5. & \cmark & \cmark & \xmark
& 7.9 & 47.1 & 9.3 & 27.9 & 27.8 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on pretraining losses on YouCook2.} 
\vspace{-0.7cm}
\label{table:pretraining}
\end{center}
\end{table}


\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccccc|ccccc}
& \multicolumn{2}{c}{Visual} & \multicolumn{2}{c|}{Speech} & \multirow{3}{*}{\small{SODA\_c}} & \multirow{3}{*}{\small{CIDEr}} & \multirow{3}{*}{\small{METEOR}} & \multirow{3}{*}{\makecell{\small{Mean} \\ \small{Recall}}} & \multirow{3}{*}{\makecell{\small{Mean} \\ \small{Precision}}} \\ 
& Features & \makecell{\small{Time} \\ \small{Encodings}} & \makecell{\small{Text} \\ \small{Tokens}} & \makecell{\small{Time} \\ \small{Tokens}} \\ 
\hline
1. & \cmark & \cmark & \xmark & \xmark
& 5.7 & 25.3 & 6.1 & 24.4 & 23.6 \\
2. & \xmark & \xmark & \cmark & \cmark
& 4.3 & 18.6 & 4.7 & 19.9 & 21.8 \\ 
3. & \cmark & \xmark & \cmark & \cmark
& 6.8 & 42.0 & 8.6 & 26.7 & 24.6 \\ 
4. & \cmark & \cmark & \cmark & \xmark
& 5.9 & 29.6 & 6.4 & 22.2 & 24.1 \\
5. & \cmark & \cmark & \cmark & \cmark
& 7.9 & 47.1 & 9.3 & 27.9 & 27.8 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Impact of modalities on YouCook2.} 
\vspace{-0.7cm}
\label{table:modalities}
\end{center}
\end{table}


\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc}
& \makecell{\small{Text} \\ \small{Initialization}} & \makecell{\small{Video-text} \\ \small{Pretraining}} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
\hline
1. & \xmark & \xmark
& 2.3 & 8.4 & 2.6 & 17.0 & 16.5 \\ 
2. & \cmark & \xmark
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3 \\ 
3. & \xmark & \cmark
& 8.8 & 51.3 & 9.8 & 29.2 & 28.5 \\ 
4. & \cmark & \cmark
& 7.9 & 47.1 & 9.3 & 27.9 & 27.8 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on language model initialization on YouCook2.} 
\vspace{-0.7cm}
\label{table:language}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc}
& Method & \makecell{\small{Video-text} \\ \small{Pretraining}} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
\hline
1. & Detect then describe & \xmark
& 3.0 & 9.7 & 3.0 & 20.2 & 19.1 \\ 
2. & Joint localization and captioning & \xmark
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3 \\ 
3. & Detect then describe & \cmark
& 8.3 & 46.1 & 9.1 & 28.0 & 25.9 \\ 
4. & Joint localization and captioning & \cmark
& 7.9 & 47.1 & 9.3 & 27.9 & 27.8 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Comparison to a detect then describe variant on YouCook2.} 
\vspace{-0.7cm}
\label{table:twostage}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{9pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|cc}
& \small{Timestamp Supervision} & \small{Video-text Pretraining} &  \small{CIDEr} & \small{METEOR} \\ 
\hline
1. & \xmark & \xmark
& X & X \\ 
2. & \cmark & \xmark
& 30.5 & 18.6 \\ 
3. & \xmark & \cmark
& X & X \\ 
4. & \cmark & \cmark
& 50.1 & 24.0 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Impact of the timestamp supervision for video paragraph captioning with learnt proposals on YouCook2.} 
\vspace{-0.7cm}
\label{table:time}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{cccc|ccccc}
& Denoising & \multicolumn{2}{c|}{Generative} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
& & \small{video-level} & \small{clip-level} & & & & \\ 
\hline
1. & \xmark & \xmark & \xmark
& 5.4 & 18.8 & 7.1 & 42.5 & 64.1 \\ 
2. & \cmark & \xmark & \xmark
& 5.6 & 28.3 & 8.0 & 51.9 & 53.0 \\ 
3. & \xmark & \cmark & \xmark
& 5.9 & 30.2 & 8.3 & 52.2 & 53.9 \\ %
4. & \cmark & \xmark & \cmark
& 5.8 & 28.9 & 8.2 & 52.5 & 53.1 \\
5. & \cmark & \cmark & \xmark
& 5.8 & 30.1 & 8.5 & 52.7 & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on pretraining losses on ActivityNet Captions.} 
\vspace{-0.7cm}
\label{table:pretraining}
\end{center}
\end{table}


\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccccc|ccccc}
& \multicolumn{2}{c}{Visual} & \multicolumn{2}{c|}{Speech} & \multirow{3}{*}{\small{SODA\_c}} & \multirow{3}{*}{\small{CIDEr}} & \multirow{3}{*}{\small{METEOR}} & \multirow{3}{*}{\makecell{\small{Mean} \\ \small{Recall}}} & \multirow{3}{*}{\makecell{\small{Mean} \\ \small{Precision}}} \\ 
& Features & \makecell{\small{Time} \\ \small{Encodings}} & \makecell{\small{Text} \\ \small{Tokens}} & \makecell{\small{Time} \\ \small{Tokens}} \\ 
\hline
1. & \cmark & \cmark & \xmark & \xmark
& 5.9 & 30.2 & 8.3 & 52.2 & 53.9 \\ 
2. & \xmark & \xmark & \cmark & \cmark
& 3.7 & 12.4 & 4.9 & 42.1 & 64.6 \\ 
3. & \cmark & \xmark & \cmark & \cmark
& 5.3 & 27.0 & 7.8 & 50.6 & 53.2 \\ 
4. & \cmark & \cmark & \cmark & \xmark
& 5.6 & 27.4 & 8.2 & 51.7 & 54.2 \\
5. & \cmark & \cmark & \cmark & \cmark
& 5.8 & 30.1 & 8.5 & 52.7 & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Impact of modalities on ActivityNet Captions.} 
\vspace{-0.7cm}
\label{table:modalities}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccccc|ccccc}
& \multicolumn{2}{c}{Input Modalities} & \multicolumn{2}{c|}{Pretraining Objectives} & \multirow{2}{*}{\small{SODA\_c}} & \multirow{2}{*}{\small{CIDEr}} & \multirow{2}{*}{\small{METEOR}} & \multirow{2}{*}{\makecell{\small{Mean} \\ \small{Recall}}} & \multirow{2}{*}{\makecell{\small{Mean} \\
\small{Precision}}} \\ 
& Visual & Speech & Generative & Denoising \\ 
\hline
1. & \cmark & \xmark & \xmark & \xmark
& 3.0 & 15.6 & 3.8 & 12.1 & 22.7 \\
2. & \cmark & \cmark & \xmark & \xmark
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3 \\ 
3. & \cmark & \xmark & \cmark & \xmark
& 5.7 & 25.3 & 6.1 & 24.4 & 23.6 \\
4. & \cmark & \cmark & \cmark & \xmark
& 2.5 & 10.3 & 3.1 & 23.1 & 12.7 \\
5. & \cmark & \cmark & \cmark & \cmark
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3} & \textbf{27.9} & \textbf{27.8} \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on input modalities and pretraining objectives.}
\vspace{-0.7cm}
\label{table:modalities}
\end{center}
\end{table}


\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc}
& \makecell{\small{Text} \\ \small{Initialization}} & \makecell{\small{Video-text} \\ \small{Pretraining}} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
\hline
1. & \xmark & \xmark
& 5.4 & 21.4 & 6.8 & 42.7 & 63.2 \\ 
2. & \cmark & \xmark
& 5.4 & 18.8 & 7.1 & 42.5 & 64.1 \\ 
3. & \xmark & \cmark
& 5.7 & 28.7 & 8.0 & 52.1 & 53.0 \\ 
4. & \cmark & \cmark
& 5.8 & 30.1 & 8.5 & 52.7 & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on language model initialization on ActivityNet Captions.} 
\vspace{-0.7cm}
\label{table:language}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{3pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc}
& Method & \makecell{\small{Video-text} \\ \small{Pretraining}} & \small{SODA\_c} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
\hline
1. & Detect then describe & \xmark
& 5.9 & 27.9 & 8.2 & 54.4 & 57.7 \\ 
2. & Joint localization and captioning & \xmark
& 5.4 & 18.8 & 7.1 & 42.5 & 64.1 \\ 
3. & Detect then describe & \cmark
& 7.4 & 36.6 & 8.2 & 54.5 & 55.5 \\ 
4. & Joint localization and captioning & \cmark
& 5.8 & 30.1 & 8.5 & 52.7 & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Comparison to a detect then describe variant on ActivityNet Captions.} 
\vspace{-0.7cm}
\label{table:twostage}
\end{center}
\end{table}

\begin{table}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{9pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|cc}
& \small{Timestamp Supervision} & \small{Video-text Pretraining} &  \small{CIDEr} & \small{METEOR} \\ 
\hline
1. & \xmark & \xmark
& X & X \\ 
2. & \cmark & \xmark
& X & X \\ 
3. & \xmark & \cmark
& X & X \\ 
4. & \cmark & \cmark
& 28.0 & 17.0 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Impact of the timestamp supervision for video paragraph captioning with learnt proposals on ActivityNet Captions.} 
\vspace{-0.7cm}
\label{table:time}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\begin{subtable}[t]{0.59\textwidth}
\begin{center}
\caption{\small Dense Video Captioning}
\setlength\tabcolsep{1pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|ccc|ccc|ccc}
& \multirow{3}{*}{Method}
& \multicolumn{3}{c|}{YouCook2 (val)}
& \multicolumn{3}{c|}{ViTT (test)}
& \multicolumn{3}{c}{ActivityNet Captions (val)} \\
& & \small{SODA\_c} & \small{CIDEr} & \small{METEOR}
& \small{SODA\_c} & \small{CIDEr} & \small{METEOR} 
& \small{SODA\_c} & \small{CIDEr} & \small{METEOR} \\
\hline
1. & MT~\cite{zhou2018end} 
& --- & 6.1 & 3.2
& --- & --- & ---
& --- & 9.3 & 5.3 \\
2. & ECHR~\cite{wang2020event}
& --- & --- & 3.8
& --- & --- & ---
& 3.2 & 14.7 & 7.2 \\
3. & PDVC~\cite{wang2021end}
& 4.4 & 22.7 & 4.7
& --- & --- & ---
& 5.4 & 29.0 & 8.0 \\
4. & UEDVC~\cite{zhang2022unifying}
& --- & --- & ---
& --- & --- & ---
& 5.5 & --- & --- \\
5. & E2ESG~\cite{zhu2022end} 
& --- & --- & 3.5
& --- & 25 & 8.1
& --- & --- & ---- \\
6. & \model{} (Ours) 
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3}
& \textbf{13.1} & \textbf{41.6} & \textbf{8.2}
& \textbf{5.8} & \textbf{30.1} & \textbf{8.5} \\
\end{tabular}
}
\end{center}
\label{table:sotac}
\end{subtable}
\hfill
\begin{subtable}[t]{0.39\textwidth}
\begin{center}
\caption{\small Event Localization}
\setlength\tabcolsep{1pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|cc|cc|cc}
& \multirow{3}{*}{Method}
& \multicolumn{2}{c|}{YouCook2 (val)}
& \multicolumn{2}{c|}{ViTT (test)}
& \multicolumn{2}{c}{ActivityNet Captions (val)} \\
& & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} 
& \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}}
& \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\
\hline
1. & PDVC~\cite{wang2021end}
& --- & ---
& --- & ---
& 55.4 & 58.1 \\
2. & UEDVC~\cite{zhang2022unifying}
& --- & ---
& --- & ---
& \textbf{59.0} & \textbf{60.3} \\
3. & E2ESG~\cite{zhu2022end} 
& 20.7 & 20.6
& 32.2 & 32.1
& --- & --- \\
6. & \model{} (Ours) 
& \textbf{27.9} & \textbf{27.8}
& \textbf{40.1} & \textbf{45.3}
& 52.7 & 53.9 \\
\end{tabular}
}
\end{center}
\label{table:sotal}
\end{subtable}
\vspace{-0.7cm}
\caption{\small Comparison to the state of the art for dense video captioning and event localization.}  
\end{center}
\vspace{-0.7cm}
\label{table:sota}
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{subtable}[t]{0.59\textwidth}
\begin{center}
\caption{\small Dense Video Captioning}
\label{table:sotac}
\vspace{-0.3cm}
\setlength\tabcolsep{1pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|ccc|ccc|ccc}
\toprule
& \multirow{3}{*}{Method}
& \multicolumn{3}{c|}{YouCook2 (val)}
& \multicolumn{3}{c|}{ViTT (test)}
& \multicolumn{3}{c}{ActivityNet Captions (val)} \\
& & \small{SODA} & \small{CIDEr} & \small{METEOR}
& \small{SODA} & \small{CIDEr} & \small{METEOR} 
& \small{SODA} & \small{CIDEr} & \small{METEOR} \\
\midrule
1. & MT~\cite{zhou2018end} 
& --- & 6.1 & 3.2
& --- & --- & ---
& --- & 9.3 & 5.3 \\
2. & ECHR~\cite{wang2020event}
& --- & --- & 3.8
& --- & --- & ---
& 3.2 & 14.7 & 7.2 \\
3. & PDVC~\cite{wang2021end}
& 4.4 & 22.7 & 4.7
& --- & --- & ---
& 5.4 & 29.0 & 8.0 \\
4. & UEDVC~\cite{zhang2022unifying}
& --- & --- & ---
& --- & --- & ---
& 5.5 & --- & --- \\
5. & E2ESG~\cite{zhu2022end} 
& --- & 25.0* & 3.5
& --- & 25.0 & 8.1
& --- & --- & ---- \\
6. & \model{} (Ours) 
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3}
& \textbf{13.5} & \textbf{43.5} & \textbf{8.5}
& \textbf{5.8} & \textbf{30.1} & \textbf{8.5} \\
\bottomrule
\end{tabular}
}
\end{center}
\end{subtable}
\hfill
\begin{subtable}[t]{0.39\textwidth}
\begin{center}
\caption{\small Event Localization}
\label{table:sotal}
\vspace{-0.1cm}
\setlength\tabcolsep{1pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|cc|cc|cc}
\toprule
& \multirow{3}{*}{Method}
& \multicolumn{2}{c|}{YouCook2 (val)}
& \multicolumn{2}{c|}{ViTT (test)}
& \multicolumn{2}{c}{\makecell{\small{ActivityNet} \\ \small{Captions (val)}}} \\
& & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} 
& \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}}
& \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\
\midrule
1. & PDVC~\cite{wang2021end}
& --- & ---
& --- & ---
& 55.4 & 58.1 \\
2. & UEDVC~\cite{zhang2022unifying}
& --- & ---
& --- & ---
& \textbf{59.0} & \textbf{60.3} \\
3. & E2ESG~\cite{zhu2022end} 
& 20.7* & 20.6*
& 32.2* & 32.1*
& --- & --- \\
4. & \model{} (Ours) 
& \textbf{27.9} & \textbf{27.8}
& \textbf{42.6} & \textbf{46.2}
& 52.7 & 53.9 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{subtable}
\vspace{-0.3cm}
\caption{\small Comparison to the SoTA for dense captioning (Table~\ref{table:sotac}) and event localization (Table~\ref{table:sotal}).
* Results provided by the authors.}  
\label{table:sota}
\end{center}
\vspace{-0.5cm}
\end{table*}

\begin{table*}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{6pt}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccc|ccccc|ccccc}
& \multicolumn{2}{c|}{Pretraining Input} &
\multicolumn{5}{c|}{YouCook2 (val)} &
\multicolumn{5}{c}{ActivityNet Captions (val)} \\
& Untrimmed & Time Tokens & \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} 
& \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\ \small{Precision}} \\ 
\hline
1. & --- & ---
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3 
& 5.4 & 18.8 & 7.1 & 42.5 & \textbf{64.1} \\ 
2. & \xmark & \xmark
& 5.5 & 27.8 & 6.5 & 21.0 & 22.9
& 5.4 & 25.5 & 7.9 & 50.4 & 54.8 \\
3. & \cmark & \xmark
& 6.7 & 35.0 & 7.3 & 22.8 & 24.7 
& 5.5 & 26.5 & 8.0 & 50.7 & 56.6 \\
4. & \cmark & \cmark
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3} & \textbf{27.9} & \textbf{27.8} 
& \textbf{5.8} & \textbf{30.1} & \textbf{8.5} & \textbf{52.7} & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on our pretraining task formulation that uses untrimmed video-speech inputs, where time information from the speech transcripts is integrated via the time tokens.}
\vspace{-0.7cm}
\label{table:pretraining}
\end{center}
\end{table*}

\begin{table*}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{4pt}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccccc|ccccc|ccccc}
& \multicolumn{2}{c}{Input Modalities} & \multicolumn{2}{c|}{Pretraining Objectives} &
\multicolumn{5}{c|}{YouCook2 (val)} &
\multicolumn{5}{c}{ActivityNet Captions (val)} \\
& Visual & Speech & Generative & Denoising & \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} 
& \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} \\ 
\hline
1. & \cmark & \xmark & \xmark & \xmark
& 3.0 & 15.6 & 3.8 & 12.1 & 22.7
& 5.4 & 16.5 & 6.9 & 38.1 & \textbf{65.2} \\
2. & \cmark & \cmark & \xmark & \xmark
& 4.0 & 18.0 & 4.6 & 17.2 & 20.3
& 5.4 & 18.8 & 7.1 & 42.5 & 64.1 \\ 
3. & \cmark & \xmark & \cmark & \xmark
& 5.7 & 25.3 & 6.1 & 24.4 & 23.6
& \textbf{5.9} & \textbf{30.2} & 8.3 & 52.2 & 53.9 \\
4. & \cmark & \cmark & \cmark & \xmark
& 2.5 & 10.3 & 3.1 & 23.1 & 12.7
& 4.8 & 17.0 & 6.2 & 42.7 & 63.0 \\
5. & \cmark & \cmark & \cmark & \cmark
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3} & \textbf{27.9} & \textbf{27.8} 
& 5.8 & 30.1 & \textbf{8.5} & \textbf{52.7} & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on input modalities and pretraining objectives.}
\vspace{-0.7cm}
\label{table:modalities}
\end{center}
\end{table*}

\begin{table*}[t]
\centering
\vspace{-0pt}
\begin{center}
\setlength\tabcolsep{6pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccc|ccccc|ccccc}
& \makecell{\small{Visual} \\
\small{Temporal Embedding}} & \makecell{\small{Speech} \\
\small{Time Tokens}}  &
\multicolumn{5}{c|}{YouCook2 (val)} &
\multicolumn{5}{c}{ActivityNet Captions (val)} \\
& & & \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} 
& \small{SODA} & \small{CIDEr} & \small{METEOR} & \makecell{\small{Mean} \\ \small{Recall}} & \makecell{\small{Mean} \\
\small{Precision}} \\ 
\hline
1. & \xmark & \xmark
& X & X & X & X & X
& X & X & X & X & X \\
2. & \cmark & \xmark
& X & X & X & X & X
& X & X & X & X & X \\
3. & \xmark & \cmark
& 6.8 & 42.0 & 8.6 & 26.7 & 24.6
& 5.3 & 27.0 & 7.8 & 50.6 & 53.2 \\ 
4. & \cmark & \cmark
& \textbf{7.9} & \textbf{47.1} & \textbf{9.3} & \textbf{27.9} & \textbf{27.8} 
& 5.8 & 30.1 & \textbf{8.5} & \textbf{52.7} & 53.9 \\ 
\end{tabular}}
\vspace{-0.4cm}
\caption{\small Ablation on the time encodings in our model.}
\vspace{-0.7cm}
\label{table:time}
\end{center}
\end{table*}
